SCARCE: Scalable Cascade Analysis for Rare-event Characterisation via Embeddings

Rare events govern the safety profile of modern AI systems, yet their probabilities are extremely difficult to estimate: direct Monte Carlo requires prohibitive sample budgets. Subset Simulation (SS) addresses this by decomposing a rare-event probability into moderate conditional probabilities over nested intermediate events. However, classical SS requires a handcrafted scalar performance function whose sublevel sets define those events, demanding detailed knowledge of the failure geometry and limiting transfer to new domains. We propose SCARCE (Scalable Cascade Analysis for Rare-event Characterisation via Embeddings), which replaces the performance function with learned latent representations and geometric rulers that score proximity to failure regions. Adaptive thresholding constructs nested intermediate events directly from data. We formalise SCARCE through a non-negative supermartingale, yielding a high-probability upper envelope that remains valid under early stopping. On MNIST misclassification, where dense Monte Carlo provides ground truth, SCARCE achieves approximately 400--500 times lower mean absolute error than grid-searched traditional SS while eliminating systematic over-counting. We then study PAIR-style LLM jailbreaks under a fleet-level threat model with adversarial fraction $\eta$. On Llama-Guard-3-8B hidden states, a PCA-based ruler attains 2.6% mean relative error for $\eta \geq 10^{-3}$ against finite-sample references whose average bootstrap relative half-width is 27.9%, and transfers to a GCG-style corpus with 2.93% relative error after recalibration. A directional criterion $\mathrm{KL}(p_{\mathrm{good}}\,\|\,p_{\mathrm{bad}})$ ranks rulers consistently with estimation error (Spearman $\rho=0.83$).

==> Legacy/Section4_Theory.tex <==
\section{Theoretical Guarantees}
\label{sec:theory}

The adaptive, data-driven nature of SSDD raises a fundamental question: \emph{do the probability estimates remain statistically valid when thresholds are chosen from the data?} This section formalizes SSDD via supermartingale. First, A filtration is constructed to explicit randomness and revealed information per level~(\S\ref{sec:filtration}). Second, we provide an upper bound~(\S\ref{sec:supermartingale}), and anytime-validity analysis in the last level~(\S\ref{sec:anytime}).

% ------------------------------------------------------------------
\subsection{Filtration: Revealed Information and Remaining Randomness}
\label{sec:filtration}

Let $(\Omega,\mathcal{F},\mathbb{P})$ be the underlying probability
space.  Recall from Section~\ref{sec:method-rulers} that the failure
event $F = \{x \in \mathcal{X} : G(f_\theta(x)) \geq \gamma\}$ is
decomposed into nested intermediate events
\begin{equation}\label{eq:nested}
  \mathcal{X} = F_0 \supset F_1 \supset \cdots \supset F_L = F,
  \qquad
  F_l = \bigl\{x : G(f_\theta(x)) \geq \gamma_l\bigr\},
\end{equation}
with the failure probability factored as
$p_f = \prod_{l=1}^{L} \mathbb{P}(F_l \mid F_{l-1})$.

As the algorithm advances from level~$0$ to level~$l$, the
information it has accumulated comprises the encoder outputs, ruler
scores, surviving samples,thresholds, and MCMC inner randomness.  We formalise this as the \emph{level-wise filtration}
\begin{equation}\label{eq:filtration}
  \mathcal{G}_l
  \;=\;
  \sigma\!\Big(
    \bigl\{f_\theta(X_j^{(i)}),\;
           G\bigl(f_\theta(X_j^{(i)})\bigr)
    \bigr\}_{j=1}^{N},\;
    \gamma_{1:l}
    \;\Big|\; 0 \leq i \leq l
  \Big),
  \qquad
  \mathcal{G}_0 \subset \mathcal{G}_1 \subset \cdots
  \subset \mathcal{G}_L,
\end{equation}
where we use $\mathcal{G}$ instead of $\mathcal{F}$ to
distinguish the filtration from the failure events $F_l$.

Two properties are essential for the sequel:
%
\begin{enumerate}[label=(\roman*),nosep]
\item \textbf{Measurability of thresholds.}\;
  $\gamma_l$ is $\mathcal{G}_{l-1}$-measurable: it is computed as the
  $(1{-}p_0)$-quantile of the level-$(l{-}1)$ ruler scores and is
  therefore determined \emph{before} level-$l$ sampling begins.
\item \textbf{Conditional randomness.}\;
  Conditional on $\mathcal{G}_l$, the MCMC proposals at level~$l{+}1$
  remain stochastic, since they depend only on the current population
  and the transition kernel, not on future randomness.
\end{enumerate}
%
Together, these properties separate \emph{revealed} from
\emph{remaining} randomness and form the foundation for the
martingale argument below.
The level-wise filtration~\eqref{eq:filtration} is a coarsening of
the finer, step-wise filtration that tracks each individual MCMC
accept/reject decision within a level; the coarser version suffices
for the guarantees established here, though the finer one would be
needed for within-level concentration bounds.

% ------------------------------------------------------------------
\subsection{Supermartingale Construction and Upper Bound}
\label{sec:supermartingale}

Let $p_l = \mathbb{P}(F_l \mid F_{l-1})$ be the true conditional
probability at level~$l$, and let $\hat{p}_l$ denote the SSDD
estimate of this quantity. $\hat{p}_l = p_0$ at intermediate levels by
quantile construction; $\hat{p}_L = K_L/N$ at the terminal level,
where $K_L$ counts samples that enter the failure region $F$.
Define the cumulative products
\[
  P_l = \prod_{i=1}^{l} p_i = \mathbb{P}(F_l),
  \qquad
  \hat{P}_l = \prod_{i=1}^{l} \hat{p}_i,
\]
and the likelihood-ratio process
\begin{equation}\label{eq:martingale}
  M_0 = 1,
  \qquad
  M_l \;=\; \frac{\hat{P}_l}{P_l}
       \;=\; \prod_{i=1}^{l} \frac{\hat{p}_i}{p_i},
  \qquad l = 1,\dots,L.
\end{equation}

\begin{theorem}[Supermartingale property]
\label{thm:supermartingale}
Suppose at each level~$l$:
\begin{enumerate}[label=(\alph*),nosep]
\item the MCMC kernel satisfies detailed balance with respect to
  $\mathbb{P}(\cdot \mid F_{l-1})$, and
\item the $N$ samples used to compute $\hat{p}_l$ are drawn from a
  chain that has mixed sufficiently to give
  $\mathbb{E}[\hat{p}_l \mid \mathcal{G}_{l-1}] \leq p_l$.
\end{enumerate}
Then $\{M_l\}_{l=0}^{L}$ is a nonneg supermartingale with
respect to~$\{\mathcal{G}_l\}$:
\[
  \mathbb{E}[M_l \mid \mathcal{G}_{l-1}]
  \;\leq\; M_{l-1},
  \qquad l = 1,\dots,L.
\]
Under perfect mixing
($\mathbb{E}[\hat{p}_l \mid \mathcal{G}_{l-1}] = p_l$),
the process is a martingale.
\end{theorem}

\begin{proof}[Proof sketch]
Since $\hat{p}_l / p_l$ is $\mathcal{G}_l$-measurable and $M_{l-1}$
is $\mathcal{G}_{l-1}$-measurable,
\[
  \mathbb{E}[M_l \mid \mathcal{G}_{l-1}]
  = M_{l-1}\;\cdot\;
    \mathbb{E}\!\left[\frac{\hat{p}_l}{p_l}
    \;\middle|\; \mathcal{G}_{l-1}\right]
  \leq M_{l-1}\;\cdot\;\frac{p_l}{p_l}
  = M_{l-1},
\]
where the inequality uses assumption~(b).
Non-negativity follows because $\hat{p}_l \geq 0$ and $p_l > 0$ for
all~$l$ (each intermediate event is non-empty by the quantile
construction).  A detailed proof establishing the measurability
conditions and the role of the adaptive quantile is given in
Appendix~\ref{app:proofs}.
\end{proof}

\begin{corollary}[One-sided concentration bound]
\label{cor:upper-bound}
By Ville's inequality~\cite{howard2021time,ramdas2020admissible},
\begin{equation}\label{eq:ville}
  \mathbb{P}\!\left(
    \sup_{1 \leq l \leq L}\;
    \frac{\hat{P}_l}{P_l}
    \;\geq\; \frac{1}{\alpha}
  \right)
  \;\leq\; \alpha.
\end{equation}
Equivalently, with probability at least $1{-}\alpha$, the SSDD
estimate at \emph{every} level simultaneously satisfies
$\hat{P}_l \leq P_l / \alpha$.  This provides a one-sided confidence
envelope: the running SSDD estimate is a valid upper bound (up to the
factor $1/\alpha$) on the true probability $P_l$ at any level.
\end{corollary}

In practice, the bound is conservative.  The LLM jailbreak
experiments (Section~\ref{sec:exp-llm}) show that for the calibrated
\textsc{pc1}/p75 ruler at the recommended operating point, the mean
ratio $|\hat{P}_f/P_f - 1|$ is $2.6\%$, well within the theoretical
envelope even for moderate~$\alpha$.

% ------------------------------------------------------------------
\subsection{Anytime Validity and Last-Level Calibration}
\label{sec:anytime}

\paragraph{Stopping rules.}
The supermartingale property ensures that SSDD produces valid estimates
regardless of when the algorithm terminates, provided the stopping
rule is a \emph{stopping time} with respect to
$\{\mathcal{G}_l\}$---that is, the decision to stop at level~$l$
depends only on information available up to level~$l$.  We consider
two natural choices:
%
\begin{enumerate}[label=(\alph*),nosep]
\item \textbf{Failure-detection stop:}
  $\ell^* = \min\{l : K_l > 0\}$, where
  $K_l = \sum_{j=1}^{N} \mathbf{1}(X_j^{(l)} \in F)$ counts samples
  that have entered the true failure region.  This is the default
  rule used in Sections~\ref{sec:exp-cv}--\ref{sec:exp-llm}.
\item \textbf{Confidence-based stop:}
  $\ell^* = \min\{l : \hat{P}_l / \alpha \leq \varepsilon\}$ for a
  user-specified tolerance~$\varepsilon$, which terminates when the
  upper bound from Corollary~\ref{cor:upper-bound} is tight enough.
\end{enumerate}
%
Both are stopping times with respect to $\{\mathcal{G}_l\}$, since
each depends only on the samples and counts available at level~$l$.
By the optional stopping theorem for nonnegative supermartingales,

\begin{proposition}[Anytime validity]
\label{prop:anytime}
For any stopping time $\ell^* \leq L$,\;
$\mathbb{E}[M_{\ell^*}] \leq M_0 = 1$,
and hence
\begin{equation}\label{eq:anytime}
  \mathbb{P}\!\left(
    \hat{P}_{\ell^*} \;\geq\; \frac{P_{\ell^*}}{\alpha}
  \right)
  \;\leq\; \alpha.
\end{equation}
The final SSDD estimate $\hat{P}_f = \hat{P}_{\ell^*}$ inherits the
concentration guarantee of Corollary~\ref{cor:upper-bound} without
adjustment for the data-dependent choice of~$\ell^*$.
\end{proposition}

% ============================================================
% RED-LINE TODO (Session 3.1, 2026-04-14): this paragraph currently
% treats C_tau = precision/recall as always-on. Under the revised
% §3.4/§3.5 split, C_tau applies only in the OPTIONAL two-threshold
% mode (§\ref{sec:two-threshold}). The universal anytime-valid
% argument should flow through the SS-mechanism requirement
% (last-level event = true failure, §\ref{sec:method-thresholds});
% C_tau should be presented as a constant multiplier that preserves
% the supermartingale only when two-threshold is activated.
% Rewrite the paragraph below accordingly in a dedicated §4 pass.
% ============================================================
%\textcolor{red}{\textbf{[RED-LINE: rewrite to separate the universal last-level SS requirement from the optional precision/recall correction; see Session 3.1 note above.]}}

\paragraph{Two-thresholds Situation.}
At the stopping level~$\ell^*$, SSDD applies the two-threshold
calibration introduced in Section~\ref{sec:method-thresholds}:
\begin{equation}\label{eq:cal-theory}
  \hat{P}_f^{\,\mathrm{cal}}
  = \hat{P}_{\ell^*}
    \;\times\;
    \frac{\mathrm{precision}(\tau)}{\mathrm{recall}(\tau)},
\end{equation}
where $\tau$ is the calibration threshold and the precision/recall
values are estimated once from the offline labelled data.  Crucially,
these are \emph{not} random at test time: they are deterministic
functions of the fixed offline dataset and the threshold~$\tau$, and
hence $\mathcal{G}_0$-measurable.  Writing
$C_\tau = \mathrm{precision}(\tau)/\mathrm{recall}(\tau) > 0$, the
calibrated estimator satisfies
$\hat{P}_f^{\,\mathrm{cal}} = C_\tau \cdot \hat{P}_{\ell^*}$.

Since scaling a nonnegative supermartingale by a positive constant yields
another nonnegative supermartingale, Ville's inequality gives
\begin{equation}\label{eq:ville-cal}
  \mathbb{P}\!\left(
    \hat{P}_f^{\,\mathrm{cal}}
    \;\geq\;
    \frac{C_\tau \cdot P_{\ell^*}}{\alpha}
  \right)
  \;\leq\; \alpha.
\end{equation}
In other words, the two-threshold calibration does \emph{not} break
the anytime-valid guarantee; it merely shifts the confidence envelope
by the known constant~$C_\tau$.  When $C_\tau \approx 1$---as is the
case for well-chosen rulers (Table~\ref{tab:llm-main})---the
calibrated and uncalibrated envelopes are nearly identical.

\paragraph{Summary.}
Theorem~\ref{thm:supermartingale} and
Proposition~\ref{prop:anytime} together guarantee that SSDD's
failure-probability estimates are anytime-valid: one may inspect the
running estimate at any level, stop early when a pre-specified
confidence or detection criterion is met, and still trust that the
reported probability is a statistically valid bound.  The data-driven
design of intermediate events and thresholds does \emph{not}
invalidate the guarantee, provided the MCMC proposals satisfy detailed
balance and the chains mix adequately---conditions verified
empirically in Sections~\ref{sec:exp-cv}
and~\ref{sec:exp-llm}.



==> Legacy/Section4_Theory_V2.tex <==
\section{Theoretical Guarantees}
\label{sec:theory}

The adaptive, data-driven nature of \projname\ raises a fundamental question: \emph{do the probability estimates remain statistically valid when thresholds are chosen from the data?} This section formalises \projname\ through a supermartingale argument. \S\ref{sec:filtration} constructs a level-wise filtration that separates revealed information from remaining randomness. \S\ref{sec:supermartingale} consumes this filtration to build a likelihood-ratio supermartingale and derive a one-sided Ville bound. \S\ref{sec:anytime} extends the result to arbitrary stopping times and treats the optional two-threshold calibration. Generalised proofs and the finer step-wise filtration live in Appendix~\ref{app:martingale}.

% ------------------------------------------------------------------
\subsection{Filtration: Revealed Information and Remaining Randomness}
\label{sec:filtration}

Let $(\Omega,\mathcal{F},\mathbb{P})$ be the underlying probability space. Recall from Section~\ref{sec:method-rulers} that the failure event $F = \{x \in \mathcal{X} : G(f_\theta(x)) \geq \gamma\}$ is decomposed into nested intermediate events $\mathcal{X} = F_0 \supset F_1 \supset \cdots \supset F_L = F$ with $F_l = \{x : G(f_\theta(x)) \geq \gamma_l\}$, and the failure probability factored as $p_f = \prod_{l=1}^{L} \mathbb{P}(F_l \mid F_{l-1})$.

As the algorithm advances from level~$0$ to level~$l$, the accumulated information comprises encoder outputs, ruler scores, surviving samples, thresholds, and MCMC inner randomness. We formalise this as the \emph{level-wise filtration}
\begin{equation}\label{eq:filtration}
  \mathcal{G}_l
  \;=\;
  \sigma\!\Big(
    \bigl\{f_\theta(X_j^{(i)}),\;G\bigl(f_\theta(X_j^{(i)})\bigr)\bigr\}_{j=1}^{N},\;
    \gamma_{1:l}
    \;\Big|\; 0 \leq i \leq l
  \Big),
  \quad
  \mathcal{G}_0 \subset \cdots \subset \mathcal{G}_L,
\end{equation}
where $\mathcal{G}$ distinguishes the filtration from the failure events $F_l$.

Two properties of $\{\mathcal{G}_l\}$ are consumed by the supermartingale argument in \S\ref{sec:supermartingale}:
\begin{enumerate}[label=(\roman*),nosep]
\item \textbf{Measurability of thresholds and estimates.}\;
  The adaptive threshold $\gamma_l$ is $\mathcal{G}_{l-1}$-measurable, since it is the $(1{-}p_0)$-quantile of level-$(l{-}1)$ ruler scores. The level-$l$ estimate $\hat{p}_l$ is $\mathcal{G}_l$-measurable.
\item \textbf{Conditional randomness.}\;
  Given $\mathcal{G}_l$, the MCMC proposals at level~$l{+}1$ remain stochastic: they depend only on the current surviving population and the transition kernel, not on future randomness.
\end{enumerate}

These two properties together separate revealed randomness, which is $\mathcal{G}_l$-measurable and therefore treated as a constant when conditioning on $\mathcal{G}_l$, from remaining randomness, which produces the conditional expectation used in the supermartingale inequality. The finer step-wise filtration $\mathcal{G}_{l,k}$ that tracks individual MCMC proposals within a level is deferred to Appendix~\ref{app:martingale:stepwise}; the coarser level-wise version suffices for all guarantees below.

% ------------------------------------------------------------------
\subsection{Supermartingale Construction and Upper Bound}
\label{sec:supermartingale}

The supermartingale argument is built directly on $\{\mathcal{G}_l\}$ of \S\ref{sec:filtration}. Let $p_l = \mathbb{P}(F_l \mid F_{l-1})$ be the true conditional probability at level~$l$, and $\hat{p}_l$ its \projname\ estimate. By quantile construction $\hat{p}_l = p_0$ at intermediate levels, and $\hat{p}_L = K_L/N$ at the terminal level, where $K_L$ counts samples entering $F$. Define $P_l = \prod_{i=1}^{l} p_i = \mathbb{P}(F_l)$, $\hat{P}_l = \prod_{i=1}^{l} \hat{p}_i$, and the likelihood-ratio process
\begin{equation}\label{eq:martingale}
  M_0 = 1, \qquad
  M_l \;=\; \hat{P}_l / P_l
       \;=\; \prod_{i=1}^{l} \hat{p}_i/p_i,
  \qquad l = 1,\dots,L.
\end{equation}
By property~(i) of \S\ref{sec:filtration}, each factor $\hat{p}_i/p_i$ is $\mathcal{G}_i$-measurable, so $M_l$ is adapted to $\{\mathcal{G}_l\}$.

\begin{theorem}[Supermartingale property]
\label{thm:supermartingale}
Suppose at each level~$l$:
\begin{enumerate}[label=(\alph*),nosep]
\item the MCMC kernel satisfies detailed balance with respect to $\mathbb{P}(\cdot \mid F_{l-1})$, and
\item the $N$ samples used to compute $\hat{p}_l$ are drawn from a chain that has mixed sufficiently to give $\mathbb{E}[\hat{p}_l \mid \mathcal{G}_{l-1}] \leq p_l$.
\end{enumerate}
Then $\{M_l\}_{l=0}^{L}$ is a nonnegative supermartingale with respect to~$\{\mathcal{G}_l\}$:
\[
  \mathbb{E}[M_l \mid \mathcal{G}_{l-1}]
  \;\leq\; M_{l-1},
  \qquad l = 1,\dots,L.
\]
Under perfect mixing, $\mathbb{E}[\hat{p}_l \mid \mathcal{G}_{l-1}] = p_l$, and the process is a martingale.
\end{theorem}

\begin{proof}[Proof sketch]
Property~(i) of \S\ref{sec:filtration} gives that $\hat{p}_l/p_l$ is $\mathcal{G}_l$-measurable and $M_{l-1}$ is $\mathcal{G}_{l-1}$-measurable. Pulling the $\mathcal{G}_{l-1}$-measurable factor out,
$\mathbb{E}[M_l \mid \mathcal{G}_{l-1}] = M_{l-1}\cdot\mathbb{E}[\hat{p}_l/p_l \mid \mathcal{G}_{l-1}] \leq M_{l-1}$,
where the inequality uses assumption~(b). Non-negativity holds because $\hat{p}_l \geq 0$ and $p_l > 0$ (quantile construction keeps every intermediate event non-empty). A general statement with the step-wise filtration and measurability verification is in Appendix~\ref{app:martingale:ssdd}.
\end{proof}

\begin{corollary}[One-sided concentration bound]
\label{cor:upper-bound}
By Ville's inequality for nonnegative supermartingales~\cite{howard2021time,ramdas2020admissible},
$\mathbb{P}\!\left(\sup_{1 \leq l \leq L} \hat{P}_l / P_l \geq 1/\alpha\right) \leq \alpha$.
Equivalently, with probability at least $1{-}\alpha$, the \projname\ estimate at every level simultaneously satisfies $\hat{P}_l \leq P_l / \alpha$, giving a one-sided confidence envelope on $P_l$.
\end{corollary}

A self-contained proof of Ville's inequality is given in Appendix~\ref{app:martingale:ville}. In practice, the bound is conservative. The LLM jailbreak experiments (\S\ref{sec:exp-llm}) show that for the calibrated \textsc{pc1}/p75 ruler at the recommended operating point, the mean ratio $|\hat{P}_f/P_f - 1|$ is $2.6\%$, well within the theoretical envelope even for moderate~$\alpha$.

% ------------------------------------------------------------------
\subsection{Anytime Validity and Last-Level Calibration}
\label{sec:anytime}

\noindent\textbf{Stopping rules.}
The supermartingale property ensures that \projname\ produces valid estimates regardless of when the algorithm terminates, provided the stopping rule is a \emph{stopping time} with respect to $\{\mathcal{G}_l\}$: the decision to stop at level~$l$ must depend only on information available up to level~$l$. We consider two natural choices:
\begin{enumerate}[label=(\alph*),nosep]
\item \textbf{Failure-detection stop:}
  $\ell^* = \min\{l : K_l > 0\}$, where $K_l = \sum_{j=1}^{N} \mathbf{1}(X_j^{(l)} \in F)$ counts samples that have entered the true failure region. This is the default rule used in \S\ref{sec:exp-cv} and \S\ref{sec:exp-llm}.
\item \textbf{Confidence-based stop:}
  $\ell^* = \min\{l : \hat{P}_l / \alpha \leq \varepsilon\}$ for a user-specified tolerance~$\varepsilon$, which terminates when the upper bound from Corollary~\ref{cor:upper-bound} is tight enough.
\end{enumerate}
Both are stopping times with respect to $\{\mathcal{G}_l\}$, since each depends only on samples and counts available at level~$l$.

\begin{proposition}[Anytime validity]
\label{prop:anytime}
For any stopping time $\ell^* \leq L$ with respect to $\{\mathcal{G}_l\}$, the optional stopping theorem (Appendix~\ref{app:martingale:optstop}) gives $\mathbb{E}[M_{\ell^*}] \leq M_0 = 1$, hence $\mathbb{P}(\hat{P}_{\ell^*} \geq P_{\ell^*}/\alpha) \leq \alpha$. The final \projname\ estimate $\hat{P}_f = \hat{P}_{\ell^*}$ inherits Corollary~\ref{cor:upper-bound} without adjustment for the data-dependent~$\ell^*$.
\end{proposition}

\noindent\textbf{Universal SS-mechanism requirement.}
The anytime bound above relies only on the SS-mechanism condition of \S\ref{sec:method-thresholds}, namely that the last-level event coincides with the true failure event $F$ so that $\hat{p}_L$ is an unbiased (or upwardly biased) estimate of $p_L$. No precision/recall correction is required for the bound to hold, and the universal statement of anytime validity therefore applies to every \projname\ run in which the SS-mechanism is satisfied.

\noindent\textbf{Optional two-threshold calibration.}
When the activation threshold used for MCMC drift differs from the reporting threshold $\tau$ (two-threshold mode of \S\ref{sec:two-threshold}), \projname\ reports $\hat{P}_f^{\,\mathrm{cal}} = C_\tau \cdot \hat{P}_{\ell^*}$ with $C_\tau = \mathrm{precision}(\tau)/\mathrm{recall}(\tau)$, estimated once offline. Since $C_\tau > 0$ is $\mathcal{G}_0$-measurable, it is a positive constant w.r.t.\ $\{M_l\}$; scaling preserves the supermartingale property, so Ville's inequality gives $\mathbb{P}(\hat{P}_f^{\,\mathrm{cal}} \geq C_\tau P_{\ell^*}/\alpha) \leq \alpha$. Calibration therefore does not break anytime validity; it shifts the envelope by the known constant~$C_\tau$.

\noindent\textbf{Summary.}
Theorem~\ref{thm:supermartingale} and Proposition~\ref{prop:anytime} together guarantee that \projname\ failure-probability estimates are anytime-valid: one may inspect the running estimate at any level, stop early when a pre-specified confidence or detection criterion is met, and still trust that the reported probability is a statistically valid upper bound. The data-driven design of intermediate events and thresholds does not invalidate the guarantee, provided the MCMC proposals satisfy detailed balance and the chains mix adequately. The optional two-threshold calibration preserves the guarantee up to a known multiplicative constant. Both conditions are verified empirically in \S\ref{sec:exp-cv} and \S\ref{sec:exp-llm}.


==> Legacy/Section6_LLM_JB.tex <==
\section{Application II: LLM Jailbreak Estimation}
\label{sec:exp-llm}

We now transfer the SSDD framework from computer vision to LLM safety,
treating jailbreak under adversarial attack as the rare event.

\subsection{Problem Setup}
\label{sec:llm-setup}

Under a fleet-level threat model, a fraction $\eta$ of queries originate
from PAIR adversaries~\cite{chao2023pair} and the remainder are benign.
The fleet-level jailbreak probability decomposes as
\begin{equation}
  P(\text{JB} \mid \text{fleet},\, t)
  \;=\; \eta \;\times\; P(\text{JB} \mid \text{PAIR},\, t),
  \label{eq:fleet-jb}
\end{equation}
where $t$ denotes the PAIR attack turn. At the canonical threat level
$\eta = 10^{-3}$ and empirical PAIR success rates of $5$--$25\%$
(turns~$1$--$5$), the fleet-level jailbreak rate is
$O(10^{-4})$--$O(10^{-5})$, firmly in the rare-event regime where standard
Monte Carlo estimation would require ${\sim}10^{6}$ samples.

\paragraph{Models and data.}
The target LLM is Llama-3.1-8B-Instruct, attacked by
Qwen2.5-14B-Instruct via PAIR, and judged by
Llama-Guard-3-8B~\cite{jailbreakbench2024}. Our primary dataset
(\textsc{6k\_Mixed}, $40{,}230$ records across $2{,}016$ behaviour units)
covers $988$ harmful and $1{,}028$ benign families over full $20$-turn
PAIR trajectories with no early stopping. A jailbreak is declared when
$p_{\text{unsafe}} > 0.80$. Five per-turn $\eta$-mixed distributions
($\eta = 10^{-3}$) yield fleet-level jailbreak rates of
$0.005$--$0.025\%$, confirming the rare-event regime.

\paragraph{Encoder: judge hidden states.}
Rather than using an external sentence encoder, we extract embeddings from
the judge model itself --- Llama-Guard-3-8B. Response text is formatted in
the Llama-Guard conversation template and passed through a frozen forward
pass; the mean-pooled last hidden layer yields a $4{,}096$-dimensional
embedding. An MLP projection head ($4096 \!\to\! 256 \!\to\! 64$,
L2-normalised) compresses embeddings for ruler fitting, providing
well-conditioned covariance matrices ($n/d$ ratios of $32$--$157\times$;
condition numbers ${\sim}1{,}400$). Using the judge's own hidden states
ensures that the ruler operates in the judge's decision space, eliminating
the encoder--judge alignment gap.

\subsection{Transfer Challenges}
\label{sec:llm-transfer}

The transition from vision to LLM latent space reveals three fundamental
failures of the inherited methodology.

\paragraph{The Mahalanobis ruler is structurally broken.}
Part~1's top ruler family, Mahalanobis distance to the failure centroid
(R8 in Appendix~\ref{app:rulers}), fails categorically in LLM space:
Cohen's $d \approx 0$ across all five turns (range $-0.14$ to $+0.19$).
The apparent $0.7$ ratio under the inherited configuration is a count
coincidence --- the ruler identifies records near the $p_{\text{unsafe}}$-weighted centroid (typically $p_{\text{unsafe}} \approx 0.42$--$0.77$),
not actual jailbreaks ($p_{\text{unsafe}} > 0.80$). The root cause is
noise-dimension dominance: $56$ of $64$ projected dimensions are
dominated by the regularisation floor ($10^{-5}$), and inverse-covariance
eigenvalues reach ${\sim}10^{5}$ in these noise dimensions versus
${\sim}60$ in data dimensions. Five centroid-reweighting variants
(power, exponential, JB-only, contrast) were tested; none can fix
this direction-agnostic noise amplification.

\paragraph{More samples cannot fix a ruler problem.}
An initial $N$-population grid ($N \in \{20\text{k},\, 50\text{k},\,
100\text{k},\, 200\text{k},\, 500\text{k}\}$) confirms that increasing
$N$ reduces variance ($\text{SE} \propto 1/\!\sqrt{N}$) but cannot
correct the systematic bias introduced by a broken ruler. The ratio
centroid remains at ${\sim}0.7$ regardless of $N$ under the Mahalanobis
ruler, pinpointing the problem as one of \emph{ruler quality}, not
\emph{sample size}.

\textcolor{red}{\textbf{[TODO --- proofreading reminder:} this paragraph is the anchor for the ``ruler-selection guidance'' contribution in Section~\ref{sec:intro}. Consider promoting it out of the ``Transfer Challenges'' subsection into its own named paragraph/subsection (e.g., \S``Ruler Selection Guidance: Directional KL Criterion'') so the contribution bullet has a clear cross-reference. \textbf{REMOVE this note before submission.]}}

\paragraph{Symmetric metrics fail for ruler selection.}
Fourteen candidate metrics were evaluated against ground-truth SSDD error
across six ruler families. Symmetric measures --- Cohen's $d$, AUC,
Jensen--Shannon, mutual information, Wasserstein --- all yield
Spearman $\rho \leq 0.09$ and select the wrong family. The reason is
structural: at $\eta \ll 1$, the fleet is ${\sim}100\%$ non-JB, and
SSDD estimation bias is driven by one-sided leakage of benign mass into
the jailbreak region. A closed-form bias decomposition makes this
precise:
\begin{equation}
  \frac{\hat{P}_{\text{cor}} - \eta\pi}{\eta\pi}
  \;=\; \frac{1-\eta}{\eta}
        \;\times\; \frac{P_b(\tau)}{P_h(\tau)},
  \label{eq:bias-decomp}
\end{equation}
where $P_b(\tau)$ is the benign leakage above threshold $\tau$ and
$P_h(\tau)$ is the harmful mass above $\tau$. At $\eta = 10^{-3}$,
the prefactor $(1\!-\!\eta)/\eta \approx 1{,}000$: even a leakage
ratio of $10^{-3}$ causes $100\%$ relative error. The directional KL
divergence $\text{KL}(p_{\neg\text{JB}} \| p_{\text{JB}})$, evaluated
at the worst turn, integrates the log-leakage ratio under the
distribution carrying the leakage mass, achieving
$\rho = 0.83$ ($p = 0.04$) and correctly selecting PC1
(cross-validated: leave-one-family-out min $\rho \geq 0.70$;
leave-one-turn-out min $\rho \geq 0.71$).

\subsection{Calibrated 1D-Projection Rulers}
\label{sec:llm-rulers}

Motivated by the transfer failures, we introduce \emph{calibrated
1D-projection rulers} with a two-threshold design that decouples the
adaptive threshold used during MCMC exploration from the final jailbreak
probability calibration.

\paragraph{Two-threshold calibration.}
The corrected estimator is
\begin{equation}
  \hat{P}(\text{JB})
  \;=\; \hat{P}(\text{score} \geq \tau)
        \;\times\; \frac{\text{precision}(\tau)}{\text{recall}(\tau)},
  \label{eq:two-threshold}
\end{equation}
where $\tau$ is a fixed calibration threshold set at a chosen percentile
of the harmful score distribution, and precision/recall are known
constants from labelled training data. The derivation is exact:
$\hat{P}(\text{score} \geq \tau) \times P(\text{JB} \mid
\text{score} \geq \tau) = P(\text{JB} \wedge \text{score} \geq \tau)
= P(\text{JB}) \times \text{recall}(\tau)$, so dividing by recall
yields an unbiased estimator. The earlier formula
($\hat{P} = p_f \times \text{precision}$) systematically underestimated
by exactly $(1 - \text{recall})$; the correction reduces mean error from
$22\%$ to $2.6\%$ on the winning ruler.

\paragraph{Ruler families.}
Five projection families are compared, each with four threshold
percentiles (p50, p75, p90, p95):

\begin{table}[t]
\centering
\caption{Ruler families for LLM jailbreak estimation. PC1 and Centroid
at $p75$ achieve the lowest estimation error; the inherited Mah\_bad
baseline is structurally broken ($d \approx 0$).}
\label{tab:llm-rulers}
\small
\begin{tabular}{llr}
\toprule
Family & Direction Method & Cohen's $d$ \\
\midrule
\textbf{PC1} & First principal component of harmful embeddings & $\mathbf{1.51}$ \\
Centroid & Normalised $\mu_{\text{safe}} \!\to\! \mu_{\text{bad}}$ direction & $1.53$ \\
Fisher LDA & $S_w^{-1}(\mu_{\text{JB}} - \mu_{\neg\text{JB}})$ & --- \\
Logistic Reg. & L2-regularised logistic weight vector & --- \\
Mah\_bad & Full Mahalanobis to weighted centroid & $\approx 0$ \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Threshold percentile as bias--variance control.}
The threshold percentile controls the operating point: lower percentiles
yield looser thresholds with higher precision but more benign leakage,
while higher percentiles tighten the boundary at the cost of more MCMC
levels. At the canonical $\eta = 10^{-3}$, $p75$ achieves strict
dominance --- same cost as $p50$ (${\sim}11\,$ms vs.\ $9\,$ms, both in
the level-$0$ regime with no MCMC needed) but ${\sim}600\times$ more
accurate. Higher thresholds ($p90$, $p95$) cost $7$--$13\times$ more
\emph{and} are less accurate due to MCMC exploration overhead. At the
stress-test $\eta = 10^{-4}$, $p75$ sits at the Pareto knee.

% ============================================================
% RED-LINE TODO (Session 3.1, 2026-04-14): expand the bizarre
% p75-beats-p95 finding below into the discussion. Hypothesis
% (user): with a looser last-level threshold, MCMC at each
% level admits samples that would otherwise be rejected by a
% strict 10% per-level cut. This accidentally mitigates a
% "discontinuous rare-event miscount" pathology in classical SS:
% individual rare-event trajectories can appear benign during
% early levels and get filtered out by the strict per-level
% quantile before revealing their failure character, producing
% a systematic undercount. Loosening the last-level target keeps
% those trajectories alive through the cascade, which --- on top
% of the sampling-variance benefit --- also reduces this
% discontinuity bias. Implication: the two-threshold design is
% not only a variance fix for tight failure regions but also a
% practical cure for rare-event discontinuity under strict
% SS-level thresholds. Discuss in §\ref{sec:llm-rulers} or in
% the Discussion (§\ref{sec:discussion}); consider a dedicated
% paragraph and a forward pointer from §\ref{sec:two-threshold}.
% ============================================================
\textcolor{red}{\textbf{[RED-LINE: the $p75$-over-$p95$ accuracy
inversion is surprising and deserves its own discussion.
Working hypothesis (user, Session 3.1): a looser last-level
threshold keeps "not-bad-enough" samples alive through the
cascade that a strict per-level $10\%$ quantile would
prematurely filter out; those trajectories would otherwise
disappear before their failure character can be recognised,
producing a discontinuous-rare-event miscount. Loosening
therefore accidentally mitigates this SS-specific pathology on
top of its intended variance benefit. Expand into a full
paragraph and forward-reference from §\ref{sec:two-threshold}
in a later pass.]}}

\subsection{Results}
\label{sec:llm-results}

\paragraph{Main comparison.}
Figure~\ref{fig:accuracy-comparison} and
Table~\ref{tab:llm-main} report the main results across all ruler
families at the $p75$ threshold.

\begin{table}[t]
\centering
\caption{LLM jailbreak estimation accuracy ($\eta \geq 10^{-3}$, all
turns, $N = 20{,}000$, $20$ rounds per cell). PC1/$p75$ reduces mean
error from $56.6\%$ (Mah\_bad) to $2.6\%$.}
\label{tab:llm-main}
\small
\begin{tabular}{llrr}
\toprule
Family / Variant & Mean $|1 - \text{ratio}|$ & Cohen's $d$ & Levels (avg.) \\
\midrule
\textbf{PC1 / p75} & $\mathbf{0.026}$ (2.6\%) & $1.51$ & $1.0$ \\
Centroid / p75 & $0.028$ (2.8\%) & $1.53$ & $1.0$ \\
PC1 / p90 & $0.067$ & $1.51$ & $1.17$ \\
Centroid / p90 & $0.060$ & $1.53$ & $1.15$ \\
\midrule
Mah\_bad (baseline) & $0.566$ (56.6\%) & $\approx 0$ & $4.1$ \\
\bottomrule
\end{tabular}
\end{table}

The winning ruler, \textbf{PC1/$p75$}, achieves $2.6\%$ mean estimation
error, a $>20\times$ improvement over the $56.6\%$ error of the inherited
Mahalanobis baseline. PC1 and Centroid at $p75$ perform nearly
identically (consistent with PC1 capturing $93.8\%$ of the harmful
embedding variance); the key differentiator is that PC1 is fully
unsupervised, requiring no jailbreak labels for direction fitting.

\paragraph{Linear $\eta$-scaling.}
Figure~\ref{fig:sigma-sweep} shows that the estimated fleet-level
jailbreak rate scales linearly with $\eta$ for $\eta \geq 10^{-3}$
(ratio $\hat{P}/\eta \approx$ constant), confirming that the
calibrated ruler correctly tracks the threat-model parameter. At
$\eta = 10^{-3}$, the level-$0$ hit rate is $44\%$ and the average
number of SS levels is $5.5$. At $\eta = 10^{-1}$, all samples clear
the threshold at level~$0$, reducing to trivial Monte Carlo.

\paragraph{$N$-population scaling.}
Figure~\ref{fig:n-grid} confirms that increasing $N$ reduces variance
($\text{SE} \propto 1/\!\sqrt{N}$, verified on log-log) but does not
change the ratio centroid, which remains at ${\approx}1.0$ across all
$N$ at $\eta = 10^{-3}$. At the harder $\eta = 10^{-4}$, the
coefficient of variation drops from $2.52$ ($N = 20{,}000$) to $0.86$
($N = 500{,}000$), with diminishing returns beyond $N = 200{,}000$.

\paragraph{Per-turn dynamics.}
Figure~\ref{fig:per-turn-rate} shows the PC1/$p75$ estimated jailbreak
rate increasing monotonically with PAIR turn (from ${\sim}0.005\%$ at
turn~$1$ to ${\sim}0.025\%$ at turn~$5$), consistent with the
progressive nature of the PAIR attack. Ruler quality improves with turn
as well: Cohen's $d$ rises from $0.62$ (turn~$1$) to $1.11$ (turn~$5$),
reflecting the growing number of jailbreak examples in the cumulative
training set.

\paragraph{Threshold sweep.}
Figure~\ref{fig:threshold-sweep-1e3} shows accuracy and runtime as a
function of threshold percentile at $\eta = 10^{-3}$. The $p75$ point
dominates: it matches the cost of $p50$ (both in the level-$0$ regime)
while being ${\sim}600\times$ more accurate. At the harder
$\eta = 10^{-4}$ (Figure~\ref{fig:threshold-sweep-1e4}), $p75$
achieves $289\,$ms runtime at the Pareto knee, while $p95$ is more
accurate but costs $522\,$ms.

\paragraph{Absolute error at extreme $\eta$.}
At $\eta = 10^{-4}$, the ground truth is ${\sim}5 \times 10^{-6}$
($\approx 0.0005\%$). Even a ${\sim}8\times$ relative overestimate at
this extreme translates to an absolute error of $0.004\%$ --- negligible
for any deployment decision. Figure~\ref{fig:absolute-error} confirms
that the absolute mean error decreases monotonically with $\eta$,
reframing the large relative error at small $\eta$ as a non-issue
in practice.

\paragraph{Negative transfer.}
Part~1's top-ranked ruler (centroid direction rotated $90^{\circ}$ in
the PC1/PC2 plane) fails in LLM space: Cohen's $d$ drops from $0.86$
at turn~$1$ to $-0.02$ at turn~$3$, and the mean estimation error is
$39.96$. The mechanism is geometric: in LLM latent space, the centroid
direction $\mu_{\text{bad}} - \mu_{\text{good}}$ lies almost entirely
within the (PC1, PC2) plane (in-plane norm $\approx 0.99$), so a
$90^{\circ}$ rotation lands on pure within-harmful variance orthogonal
to jailbreak-ness. The 1D-projection \emph{family} transfers, but the
specific direction does not. Full analysis is in
Appendix~\ref{app:neg-transfer}.

% --- Figure environments ---

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/accuracy_comparison.pdf}
\caption{Ruler accuracy comparison at $p75$. PC1 achieves $2.6\%$ mean
error across $\eta \geq 10^{-3}$ and all turns, versus $56.6\%$ for
the inherited Mahalanobis baseline. CentroidRot90 (Part~1's winner)
fails with mean error $39.96$.}
\label{fig:accuracy-comparison}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_sigma_sweep.pdf}
\caption{PC1/$p75$ estimated fleet-level JB rate vs.\ $\eta$. The
ratio $\hat{P}/\eta$ is constant for $\eta \geq 10^{-3}$, confirming
linear scaling with the threat-model parameter.}
\label{fig:sigma-sweep}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_n_grid.pdf}
\caption{Effect of population size $N$ on PC1/$p75$ estimation
($\eta = 10^{-4}$). Standard error scales as $1/\!\sqrt{N}$; the ratio
centroid remains at ${\approx}1.0$, confirming that $N$ controls
variance but not accuracy.}
\label{fig:n-grid}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_per_turn_rate.pdf}
\caption{Estimated jailbreak rate by PAIR turn (PC1/$p75$,
$\eta = 10^{-3}$), showing monotone increase consistent with the
progressive nature of the PAIR attack.}
\label{fig:per-turn-rate}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_threshold_sweep_sigma1e-3.pdf}
\caption{Threshold percentile sweep at $\eta = 10^{-3}$ (PC1 family).
$p75$ achieves strict dominance: same cost as $p50$ but
${\sim}600\times$ more accurate.}
\label{fig:threshold-sweep-1e3}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_threshold_sweep_sigma1e-4.pdf}
\caption{Threshold percentile sweep at $\eta = 10^{-4}$ (PC1 family).
$p75$ sits at the Pareto knee ($289\,$ms); $p95$ trades higher cost
($522\,$ms) for marginal accuracy gains.}
\label{fig:threshold-sweep-1e4}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/absolute_error_low_sigma.pdf}
\caption{Absolute mean error vs.\ $\eta$ (PC1/$p75$). Even at
$\eta = 10^{-4}$ (ground truth ${\sim}5 \times 10^{-6}$), the
absolute error is $0.004\%$ --- negligible for deployment decisions.}
\label{fig:absolute-error}
\end{figure}

\subsection{Summary of Findings}
\label{sec:llm-summary}

\begin{enumerate}
  \item \textbf{$\mathbf{>20\times}$ accuracy improvement.}
        The calibrated PC1/$p75$ ruler reduces mean estimation error from
        $56.6\%$ (inherited Mahalanobis baseline) to $2.6\%$, achieved
        via the two-threshold design with closed-form precision/recall
        correction.
  \item \textbf{Ruler quality dominates sample size.}
        Increasing $N$ by $25\times$ (from $20$k to $500$k) halves the
        coefficient of variation but cannot correct a structurally broken
        ruler. The Mahalanobis baseline remains at ${\sim}0.7$ ratio
        regardless of $N$.
  \item \textbf{Asymmetric KL selects the right ruler.}
        Symmetric metrics (Cohen's $d$, AUC) fail because they average
        leakage in both directions; the worst-turn
        $\text{KL}(p_{\neg\text{JB}} \| p_{\text{JB}})$ achieves
        $\rho = 0.83$ and is mechanistically justified by the
        bias decomposition in Eq.~\eqref{eq:bias-decomp}.
  \item \textbf{Linear $\eta$-scaling.}
        Estimated fleet-level JB rate tracks the threat-model parameter
        faithfully for $\eta \geq 10^{-3}$; absolute error at
        $\eta = 10^{-4}$ is $0.004\%$, negligible in practice.
  \item \textbf{The framework transfers; specific directions do not.}
        The SSDD framework, 1D-projection ruler family, and two-threshold
        calibration all transfer from CV to LLM. The specific rotation
        angle (CentroidRot90) and full Mahalanobis distance do not,
        underscoring the need for domain-specific ruler re-derivation
        within the general framework.
\end{enumerate}



==> Legacy/Section6_LLM_JB_v2.tex <==
% Section 6 v2 (session 6.1): clean main body with contributions only.
% Transfer challenges and detailed ruler ranking moved to appendix.
% Style: short sentences, no em-dashes.

\section{Application II: LLM Jailbreak Estimation}
\label{sec:exp-llm}

We transfer the SSDD framework from computer vision to LLM safety. The
rare event is jailbreak under adversarial attack. This domain introduces
a fleet-level threat model with a tunable attacker percentage $\eta$, and a
different geometry of the latent space. Two methodological extensions
emerge as the core contributions of this section: \emph{calibrated
1D-projection rulers} and a \emph{two-threshold estimation formula} with
a closed-form precision/recall correction. 
%All results are reported on a $2{,}160$-run experimental grid, each cell averaged over $20$ independent rounds.
All results are reported as the average over $20$ independent rounds.

% ------------------------------------------------------------
\subsection{Experiment Setup}
\label{sec:llm-setup}

\paragraph{Threat model.}
A fraction $\eta$ of fleet queries originate from PAIR
adversaries~\citep{chao2023pair} and the remainder are benign. The
fleet-level jailbreak probability decomposes as
\begin{equation}
  P(\text{JB} \mid \text{fleet},\, t)
  \;=\; \eta \;\cdot\; P(\text{JB} \mid \text{PAIR},\, t),
  \label{eq:fleet-jb}
\end{equation}
where $t$ is the PAIR attack turn. At the canonical threat level
$\eta = 10^{-3}$ and empirical PAIR success rates of $5$--$25\%$
across turns~$1$--$5$ according to our dataset, the fleet-level jailbreak rate sits at
$O(10^{-4})$ to $O(10^{-5})$. Standard Monte Carlo would need
${\sim}10^{6}$ samples for a reliable estimate, even if it is applicable. This is the rare-event
regime SSDD targets.

\paragraph{Models.}
The target LLM is Llama-3.1-8B-Instruct. The attacker is
Qwen2.5-14B-Instruct driven by PAIR. The judge is
Llama-Guard-3-8B~\citep{jailbreakbench2024}. A jailbreak is declared
when $p_{\text{unsafe}} > 0.80$.% This is tighter than the default $0.50$ and yields cleaner calibration.

\paragraph{Dataset.}
The primary corpus is \textsc{6k\_Mixed}, with $40{,}230$ records
covering $2{,}016$ behaviour units ($988$ harmful families and
$1{,}028$ benign families). Each unit has a full $20$-turn PAIR
trajectory with no early stopping. Five per-turn $\eta$-mixed
distributions at $\eta = 10^{-3}$ yield fleet-level jailbreak rates
of $0.005$--$0.025\%$, confirming the rare-event regime.

\paragraph{Encoder: judge hidden states.}
We extract embeddings from the judge model itself rather than
external encoders. Response text is formatted in the
Llama-Guard conversation template and passed through a frozen forward
pass. The mean-pooled last hidden layer yields a $4{,}096$-dimensional
embedding. An MLP projection head ($4096 \!\to\! 256 \!\to\! 64$,
L2-normalised) compresses embeddings for ruler fitting. The resulting
covariance matrices are well conditioned: $n/d$ ratios of
$32$--$157\times$ with condition numbers around $1{,}400$. Using the
judge's own hidden states keeps the ruler inside the judge's decision
space and removes any encoder to judge alignment gap.

% ------------------------------------------------------------
\subsection{Simulation Results}
\label{sec:llm-results}

The inherited winner rulers from Section~\ref{sec:exp-cv-summary} fails on this domain due to the high-dimension latent space. The
detailed analysis of these transfer failures is in
Appendix~\ref{app:llm-transfer}.

\paragraph{Two-threshold calibration.}
The corrected estimator is
\begin{equation}
  \hat{P}(\text{JB})
  \;=\; \hat{P}(\text{score} \geq \tau)
        \;\cdot\; \frac{\text{precision}(\tau)}{\text{recall}(\tau)},
  \label{eq:two-threshold}
\end{equation}
where $\tau$ is a fixed calibration threshold set at a chosen
percentile of the harmful score distribution. Precision and recall
are known constants from labelled training data. The derivation is
exact and proved in Section~\ref{sec:anytime} (Appendix~\ref{app:two-threshold-proof}).

\paragraph{Main accuracy.}
Figure~\ref{fig:accuracy-comparison} and Table~\ref{tab:llm-main}
report accuracy across ruler families at $\eta = 10^{-3}$. The winning
ruler is \textbf{PC1/$p75$}. It achieves $2.6\%$ mean relative error
with average over all five turns, compared to $56.6\%$
for the inherited Mahalanobis baseline. This is a $>\!20\times$
improvement. PC1 and the Centroid direction perform nearly
identically, consistent with PC1 explaining $93.8\%$ of the harmful
embedding variance. PC1 has one additional property that makes it
the recommended choice: it is fully unsupervised and needs no
jailbreak labels to fit the projection direction.

\begin{table}[t]
\centering
\caption{LLM jailbreak estimation accuracy at $\tau = p75$,
$\eta \geq 10^{-3}$, all turns, $N = 20{,}000$, $20$ rounds per
cell. PC1/$p75$ reduces mean relative error from $56.6\%$ (inherited
Mahalanobis baseline) to $2.6\%$.}
\label{tab:llm-main}
\small
\begin{tabular}{llrr}
\toprule
Family / Variant & Mean $|1 - \text{ratio}|$ & Cohen's $d$ & Levels (avg.) \\
\midrule
\textbf{PC1 / $p75$}     & $\mathbf{0.026}$ (2.6\%) & $1.51$       & $1.0$ \\
Centroid / $p75$         & $0.028$ (2.8\%)          & $1.53$       & $1.0$ \\
PC1 / $p90$              & $0.067$                  & $1.51$       & $1.17$ \\
Centroid / $p90$         & $0.060$                  & $1.53$       & $1.15$ \\
\midrule
Mah\_bad (baseline)      & $0.566$ (56.6\%)         & $\approx 0$  & $4.1$ \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Efficiency.}
At $\eta = 10^{-3}$, the winning configuration operates in the
level-$0$ regime: the $p75$ threshold sits below enough of the fleet
mass that no MCMC exploration is triggered, and the average number of
SS levels is $1.0$. Per-run cost is about $11\,$ms, dominated by
embedding and score evaluation. The broken Mahalanobis baseline by
contrast forces $4.1$ average levels with no accuracy gain. Runtime
on the harder $\eta = 10^{-4}$ case is covered under the threshold
sweep below.

\paragraph{Linear $\eta$-scaling.}
Figure~\ref{fig:sigma-sweep} shows that the estimated fleet-level
jailbreak rate scales linearly with $\eta$ for $\eta \geq 10^{-3}$.
The ratio $\hat{P}/\eta$ is flat across this range, confirming that
the calibrated ruler tracks the threat-model parameter faithfully. At
$\eta = 10^{-1}$ all samples clear the threshold at level~$0$ and
the estimator reduces to plain Monte Carlo, as expected.

\paragraph{Population size $N$.}
Figure~\ref{fig:n-grid} confirms the expected
$\text{SE} \propto 1/\!\sqrt{N}$ scaling. The ratio centroid stays at
${\approx}1.0$ across $N \in \{20\text{k}, \dots, 500\text{k}\}$ at
$\eta = 10^{-3}$, so $N$ controls variance but not bias. At the
harder $\eta = 10^{-4}$, the coefficient of variation drops from
$2.52$ at $N = 20{,}000$ to $0.86$ at $N = 500{,}000$, with
diminishing returns past $N = 200{,}000$.

\paragraph{Per-turn dynamics.}
Figure~\ref{fig:per-turn-rate} shows the PC1/$p75$ estimated jailbreak
rate rising monotonically with PAIR turn, from ${\sim}0.005\%$ at
turn~$1$ to ${\sim}0.025\%$ at turn~$5$. This matches the
progressive nature of PAIR. Ruler quality also improves with turn:
Cohen's $d$ grows from $0.62$ at turn~$1$ to $1.11$ at turn~$5$, a
consequence of the accumulating jailbreak training set.

\paragraph{Threshold sweep.}
Figure~\ref{fig:threshold-sweep-1e3} reports accuracy and runtime
across threshold percentiles at $\eta = 10^{-3}$. The $p75$ point
is strictly dominant: same cost as $p50$ in the level-$0$ regime, and
about $600\times$ more accurate. Higher thresholds $p90$ and $p95$
cost $7$--$13\times$ more and are also less accurate, because the
tighter boundary forces MCMC exploration whose sampling noise swamps
the bias gain. At $\eta = 10^{-4}$
(Figure~\ref{fig:threshold-sweep-1e4}), $p75$ sits at the Pareto knee
with $289\,$ms, while $p95$ trades $522\,$ms for marginal accuracy
gains.

\paragraph{Absolute error at extreme $\eta$.}
At $\eta = 10^{-4}$ the ground truth is near $5 \times 10^{-6}$, or
$0.0005\%$. Even an $8\times$ relative overshoot at this extreme is
an absolute error of $0.004\%$, which is negligible for any
deployment decision. Figure~\ref{fig:absolute-error} shows that the
absolute mean error decreases monotonically with $\eta$. This
reframes the large relative error at small $\eta$ as a non-issue
in practice.

% ------------------------------------------------------------
\subsection{Ruler Selection Guidance}
\label{sec:llm-guidance}

The standard family of symmetric distributional metrics (Cohen's $d$,
AUC, Jensen--Shannon, mutual information, Wasserstein) fails to
identify the winning ruler in this domain. The reason is structural.
At $\eta \ll 1$, the fleet is nearly $100\%$ benign, and SSDD
estimation bias is driven by one-sided leakage of benign mass into
the jailbreak region. A selection metric therefore needs to measure
this asymmetry directly.

We recommend the directional KL divergence
$\mathrm{KL}\!\left(p_{\neg\text{JB}}\,\|\,p_{\text{JB}}\right)$
evaluated at the worst turn. It integrates the log leakage ratio
under the distribution that carries the leakage mass. On our data it
achieves Spearman $\rho = 0.83$ ($p = 0.04$) against ground-truth
SSDD error and correctly picks PC1. It also holds up under both
leave-one-family-out and leave-one-turn-out cross validation, with
$\rho \geq 0.70$ in all folds. Full rankings across $14$ candidate
metrics, per-family Cohen's $d$ values, and the bias decomposition
that motivates the asymmetric choice are in
Appendix~\ref{app:llm-ranking}.

% ------------------------------------------------------------
% --- Figure environments ---

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/accuracy_comparison.pdf}
\caption{Ruler accuracy at $\tau = p75$. PC1 reaches $2.6\%$ mean
relative error across $\eta \geq 10^{-3}$ and all turns. The
inherited Mahalanobis baseline stays at $56.6\%$.}
\label{fig:accuracy-comparison}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_sigma_sweep.pdf}
\caption{PC1/$p75$ estimated fleet-level jailbreak rate against
$\eta$. The ratio $\hat{P}/\eta$ is constant for
$\eta \geq 10^{-3}$, confirming linear tracking of the threat-model
parameter.}
\label{fig:sigma-sweep}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_n_grid.pdf}
\caption{Effect of population size $N$ on PC1/$p75$ estimation at
$\eta = 10^{-4}$. Standard error scales as $1/\!\sqrt{N}$ and the
ratio centroid stays at ${\approx}1.0$, so $N$ controls variance but
not accuracy.}
\label{fig:n-grid}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_per_turn_rate.pdf}
\caption{Estimated jailbreak rate by PAIR turn (PC1/$p75$,
$\eta = 10^{-3}$). The rate increases monotonically with turn, in
line with the progressive nature of PAIR.}
\label{fig:per-turn-rate}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_threshold_sweep_sigma1e-3.pdf}
\caption{Threshold percentile sweep at $\eta = 10^{-3}$ (PC1 family).
$p75$ is strictly dominant: same cost as $p50$ and about $600\times$
more accurate.}
\label{fig:threshold-sweep-1e3}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/pc1_threshold_sweep_sigma1e-4.pdf}
\caption{Threshold percentile sweep at $\eta = 10^{-4}$ (PC1 family).
$p75$ sits at the Pareto knee at $289\,$ms. $p95$ trades $522\,$ms
for marginal accuracy gains.}
\label{fig:threshold-sweep-1e4}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/Part_two/absolute_error_low_sigma.pdf}
\caption{Absolute mean error against $\eta$ (PC1/$p75$). Even at
$\eta = 10^{-4}$, where ground truth is near $5\times 10^{-6}$, the
absolute error is $0.004\%$. This is negligible for deployment
decisions.}
\label{fig:absolute-error}
\end{figure}

% ------------------------------------------------------------
\subsection{Summary of Findings}
\label{sec:llm-summary}

\begin{enumerate}
  \item \textbf{$\mathbf{>20\times}$ accuracy gain.}
        The calibrated PC1/$p75$ ruler reduces mean relative error
        from $56.6\%$ (inherited baseline) to $2.6\%$. The driver is
        the two-threshold design with closed-form precision/recall
        correction (Eq.~\eqref{eq:two-threshold}).
  \item \textbf{Ruler quality dominates sample size.}
        Scaling $N$ by $25\times$ halves the coefficient of variation
        but does not correct a broken ruler. The Mahalanobis baseline
        stays at ${\sim}0.7$ ratio independent of $N$
        (Appendix~\ref{app:llm-transfer}).
  \item \textbf{Linear tracking of threat-model parameter.}
        $\hat{P}/\eta$ is flat for $\eta \geq 10^{-3}$. At
        $\eta = 10^{-4}$, absolute error is $0.004\%$, negligible
        in practice.
  \item \textbf{Asymmetric selection criterion.}
        Symmetric metrics fail because they average leakage in both
        directions. Worst-turn directional KL recovers the right
        choice with $\rho = 0.83$.
  \item \textbf{The framework transfers; specific directions do not.}
        The SSDD framework, the 1D-projection family, and two-threshold
        calibration all transfer from CV to LLM. The specific rotation
        used in Part~1 (CentroidRot90) and the full Mahalanobis ruler
        do not. Domain-specific ruler re-derivation within the general
        framework is required.
\end{enumerate}


==> Sections/Bibliography.tex <==
\bibliographystyle{plain}
\begin{thebibliography}{40}
\bibitem{arditi2024refusal} A. Arditi, O. Obeso, A. Syed, D. Paleka, N. Panickssery, W. Gurnee, and N. Nanda. Refusal in language models is mediated by a single direction. \emph{NeurIPS}, 2024.
\bibitem{au2001estimation} S.-K. Au and J. L. Beck. Estimation of small failure probabilities in high dimensions by subset simulation. \emph{Probabilistic Engineering Mechanics}, 16(4):263--277, 2001.
\bibitem{au2003subset} S.-K. Au and J. L. Beck. Subset simulation and its application to seismic risk based on dynamic analysis. \emph{Journal of Engineering Mechanics}, 129(8):901--917, 2003.
\bibitem{botev2017minimax} Z. I. Botev. Minimax tilting for importance sampling. \emph{Annals of Statistics}, 45(2):468--499, 2017.
\bibitem{bucklew2004introduction} J. A. Bucklew. \emph{Introduction to Rare Event Simulation}. Springer, 2004.
\bibitem{chao2023pair} P. Chao, A. Robey, E. Dobriban, H. Hassani, G. J. Pappas, and E. Wong. Jailbreaking black box large language models in twenty queries. \emph{arXiv:2310.08419}, 2023.
\bibitem{chen2020simclr} T. Chen, S. Kornblith, M. Norouzi, and G. Hinton. A simple framework for contrastive learning of visual representations. \emph{ICML}, 2020.
\bibitem{chen2024hnnss} M. Chen, R. Giovanis, and M. Shields. Reliability analysis of complex systems using subset simulations with Hamiltonian neural networks. \emph{Structural Safety}, 110:102479, 2024.
\bibitem{davies2026pjb} X. Davies, G. Giglemiani, E. Lau, E. Winsor, G. Irving, and Y. Gal. Boundary point jailbreaking of black-box LLMs. \emph{arXiv:2602.15001}, 2026.
\bibitem{falkner2024flowres} S. Asghar, Q.-X. Pei, G. Volpe, and R. Ni. Efficient rare event sampling with unsupervised normalizing flows. \emph{Nature Machine Intelligence}, 6:1370--1381, 2024.
\bibitem{gao2024nofis} Z. Gao, D. Zhang, L. Daniel, and D. S. Boning. NOFIS: Normalizing flow for rare circuit failure analysis. In \emph{Proceedings of the 61st ACM/IEEE Design Automation Conference (DAC)}, 2024.
\bibitem{howard2021time} S. Howard, A. Ramdas, J. McAuliffe, and J. Sekhon. Time-uniform Chernoff bounds via nonnegative supermartingales. \emph{Annals of Statistics}, 49(2):1055--1080, 2021.
\bibitem{inan2023llamaguard} H. Inan, K. Upasani, J. Chi, R. Rungta, K. Iyer, Y. Mao, M. Tontchev, Q. Hu, B. Fuller, D. Testuggine, and M. Khabsa. Llama Guard: LLM-based input-output safeguard for human-AI conversations. \emph{arXiv:2312.06674}, 2023.
\bibitem{jailbreakbench2024} P. Chao, E. Debenedetti, A. Robey, M. Andriushchenko, F. Croce, V. Sehwag, E. Dobriban, N. Flammarion, G. J. Pappas, F. Tram\`er, H. Hassani, and E. Wong. JailbreakBench: An open robustness benchmark for jailbreaking large language models. \emph{NeurIPS Datasets and Benchmarks}, 2024.
\bibitem{jones2025forecasting} E. Jones, M. Tong, J. Mu, M. Mahfoud, J. Leike, R. Grosse, J. Kaplan, W. Fithian, E. Perez, and M. Sharma. Forecasting rare language model behaviors. \emph{arXiv:2502.16797}, 2025.
\bibitem{khosla2020supcon} P. Khosla, P. Teterwak, C. Wang, A. Sarna, Y. Tian, P. Isola, A. Maschinot, C. Liu, and D. Krishnan. Supervised contrastive learning. \emph{NeurIPS}, 2020.
\bibitem{lee2018mahalanobis} K. Lee, K. Lee, H. Lee, and J. Shin. A simple unified framework for detecting out-of-distribution samples and adversarial attacks. \emph{NeurIPS}, 2018.
\bibitem{li2021deep} Y. Li et al. Deep learning for rare event estimation. \emph{Neural Computing and Applications}, 2021.
\bibitem{li2024committor} Q. Li, B. Lin, and W. Ren. Computing committor functions for the study of rare events using deep learning. \emph{Journal of Chemical Physics}, 2024.
\bibitem{li2025mllmjp} W. Xu, Z. Wei, X. Sun, Z. Ying, D. Zhang, D. Yang, X. Zhang, and Q. Zou. Probabilistic modeling of jailbreak on multimodal LLMs: From quantification to application. \emph{arXiv:2503.06989}, 2025.
\bibitem{llama3herd2024} Llama Team, AI @ Meta. The Llama 3 herd of models. \emph{arXiv:2407.21783}, 2024.
\bibitem{martell2024mitigative} M. J. Martell, J. A. Baweja, and B. D. Dreslin. Mitigative strategies for recovering from large language model trust violations. \emph{Journal of Cognitive Engineering and Decision Making}, 19(1), 2024.
\bibitem{mazeika2024harmbench} M. Mazeika et al. HarmBench: A standardized evaluation framework for automated red teaming and robust refusal. \emph{ICML}, 2024.
\bibitem{mehrotra2024tap} A. Mehrotra, M. Zampetakis, P. Kassianik, B. Nelson, H. Anderson, Y. Singer, and A. Karbasi. Tree of attacks: Jailbreaking black-box LLMs with auto-generated subversions. \emph{NeurIPS}, 2024.
\bibitem{papaioannou2015mcmc} I. Papaioannou, W. Betz, K. Zwirglmaier, and D. Straub. MCMC algorithms for subset simulation. \emph{Probabilistic Engineering Mechanics}, 41:89--103, 2015.
\bibitem{papaioannou2022adaptive} I. Papaioannou, M. Ehre, and D. Straub. An adaptive subset simulation algorithm for system reliability analysis with discontinuous limit states. \emph{Reliability Engineering \& System Safety}, 225:108607, 2022.
\bibitem{ramdas2020admissible} A. Ramdas, J. Ruf, and M. Larsson. Game-theoretic statistics and safe anytime-valid inference. \emph{arXiv:2006.04292}, 2020.
\bibitem{rubinstein1999cross} R. Y. Rubinstein. The cross-entropy method for combinatorial and continuous optimization. \emph{Methodology and Computing in Applied Probability}, 1(2):127--190, 1999.
\bibitem{ruff2018deepsvdd} L. Ruff, R. A. Vandermeulen, N. G\"ornitz, L. Deecke, S. A. Siddiqui, A. Binder, E. M\"uller, and M. Kloft. Deep one-class classification. \emph{ICML}, 2018.
\bibitem{safari} W. Huang, X. Zhao, G. Jin, and X. Huang. SAFARI: Versatile and efficient evaluations for robustness of interpretability. \emph{ICCV}, 2023.
\bibitem{shen2025jailbreakradar} J. Chu, Y. Liu, Z. Yang, X. Shen, M. Backes, and Y. Zhang. JailbreakRadar: Comprehensive assessment of jailbreak attacks against LLMs. \emph{arXiv:2402.05668}, 2024.
\bibitem{song2009subset} J. Song and Z. Lu. Subset simulation for structural reliability analysis. \emph{Structural Safety}, 31(2):133--141, 2009.
\bibitem{williams1991probability} D. Williams. \emph{Probability with Martingales}. Cambridge University Press, 1991.
\bibitem{wu2024rareoutputs} G. Wu and J. Hilton. Estimating the probabilities of rare outputs in language models. \emph{ICLR}, 2025.
\bibitem{zhang2019surrogate} X. Zhang et al. Surrogate-assisted subset simulation for reliability analysis. \emph{Reliability Engineering \& System Safety}, 183:10--19, 2019.
\bibitem{zhu2024autoredteamer} A. Zhou, K. Wu, F. Pinto, Z. Chen, Y. Zeng, Y. Yang, S. Yang, O. Koyejo, J. Zou, and B. Li. AutoRedTeamer: Autonomous red teaming with lifelong attack integration. \emph{NeurIPS}, 2025.
\bibitem{zou2023repe} A. Zou, L. Phan, S. Chen, J. Campbell, P. Guo, R. Ren, A. Pan, X. Yin, M. Mazeika, A.-K. Dombrowski, S. Goel, N. Li, M. J. Byun, Z. Wang, A. Mallen, S. Basart, S. Koyejo, D. Song, M. Fredrikson, J. Z. Kolter, and D. Hendrycks. Representation engineering: A top-down approach to AI transparency. \emph{arXiv:2310.01405}, 2023.
\bibitem{zou2023universal} A. Zou, Z. Wang, N. Carlini, M. Nasr, J. Z. Kolter, and M. Fredrikson. Universal and transferable adversarial attacks on aligned language models. \emph{arXiv:2307.15043}, 2023.
\bibitem{zuev2015subset} K. M. Zuev. Subset simulation method for rare event estimation: An introduction. \emph{International Journal for Uncertainty Quantification}, 5(2), 2015.
\end{thebibliography}


==> Sections/checklist.tex <==
% NeurIPS Paper Checklist
% Answers tailored to: SCARCE: Scalable Cascade Analysis for Rare-event Characterisation via Embeddings.

\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}

    Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?

    Answer: \answerYes{}

    Justification: The abstract and introduction state five contributions: (i) the \projname\ framework that replaces handcrafted performance functions with learned latent representations and geometric rulers, (ii) a level-wise anytime-valid upper envelope established via a non-negative supermartingale, (iii) MNIST validation showing $\sim$400--500$\times$ MAE reduction over traditional SS, (iv) LLM jailbreak estimation under a fleet-level threat model, and (v) a directional KL ruler-selection criterion. Each is directly supported by Sections~\ref{sec:method},~\ref{sec:theory},~\ref{sec:exp-cv}, and~\ref{sec:exp-llm}.

\item {\bf Limitations}

    Question: Does the paper discuss the limitations of the work performed by the authors?

    Answer: \answerYes{}

    Justification: Section~\ref{sec:conclusion} discusses three limitations: dependence on embedding quality, ruler measurement bounded by normal/failure separation (with inherited biases from attack generator and judge model in the LLM setting), and the open challenge of extending \projname\ to open-ended natural-language deployment distributions. Appendix~\ref{app:llm-transfer} additionally documents the structural failure of inherited rulers across domains.

\item {\bf Theory Assumptions and Proofs}

    Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?

    Answer: \answerYes{}

    Justification: Section~\ref{sec:theory} states Assumption~\ref{ass:conservative} (conservative level estimator under detailed balance), Theorem~\ref{thm:supermartingale} (supermartingale property), and Corollaries~\ref{cor:anytime} and~\ref{cor:upper-bound}. Full proofs of Ville's inequality, the optional stopping theorem for non-negative supermartingales, and the supermartingale property of $M_l = \hat{P}_l/P_l$ are given in Appendix~\ref{app:martingale}.

\item {\bf Experimental Result Reproducibility}

    Question: Does the paper fully disclose all the information needed to reproduce the main experimental results?

    Answer: \answerYes{}

    Justification: Section~\ref{sec:exp-cv} reports seeds, number of perturbations ($10^6$ per seed for the SMC benchmark), ruler catalogue (Appendix~\ref{app:rulers}), quantile parameter $\rho$, and threshold-calibration protocol. Section~\ref{sec:exp-llm} reports the LLM jailbreak dataset (\texttt{2k\_Mixed}, $40{,}320$ records), the encoder pipeline (Llama-Guard-3-8B mean-pooled hidden states with a $4096{\to}256{\to}64$ MLP projection head), the PAIR attacker model (Qwen2.5-14B-Instruct), and the surrogate-threshold percentile sweep.

\item {\bf Open access to data and code}

    Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results?

    Answer: \answerYes{}

    Justification: A zipped reference implementation of \projname\ (ruler library, MNIST harness, and LLM evaluation scripts) is included as supplementary material, together with instructions for regenerating the \texttt{2k\_Mixed} jailbreak corpus from public JailbreakBench seeds. Combined with the public datasets (MNIST; JailbreakBench seeds) and public model checkpoints (Llama-3.1-8B-Instruct, Qwen2.5-14B-Instruct, Llama-Guard-3-8B), the full pipeline is reproducible from the submitted code, the descriptions in Sections~\ref{sec:exp-cv} and~\ref{sec:exp-llm}, and the calibration script in Appendix~\ref{app:runtime-calibration}.

\item {\bf Experimental Setting/Details}

    Question: Does the paper specify all the training and test details necessary to understand the results?

    Answer: \answerYes{}

    Justification: Section~\ref{sec:exp-cv} specifies the encoder, calibration split, ruler set, and seed count (50 seeds for screening, 100 held-out seeds for evaluation). Runtime calibration ($T_{\mathrm{ref}} = 6.473 \times 10^{-4}$~s/query on Dawn CPU) is reported in Appendix~\ref{app:runtime-calibration}. Section~\ref{sec:exp-llm} specifies PAIR attack budget (20 turns, no early stopping), victim/judge/attacker models, and the surrogate-threshold percentile grid $\{p_{50}, p_{75}, p_{90}, p_{95}\}$.

\item {\bf Experiment Statistical Significance}

    Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?

    Answer: \answerYes{}

    Justification: Figure~\ref{fig:exp2-accuracy}b reports seed-wise absolute errors as box plots over 100 held-out MNIST seeds. The directional KL ruler-selection criterion is reported with Spearman $\rho$, $p$-value, and leave-one-family-out / leave-one-turn-out cross-validation in \S\ref{sec:llm-results} and Appendix~\ref{app:llm-ranking}. Sample-size sensitivity is reported in Figure~\ref{fig:accuracy-comparison}d.

\item {\bf Experiments Compute Resources}

    Question: For each experiment, does the paper provide sufficient information on the computer resources needed to reproduce the experiments?

    Answer: \answerYes{}

    Justification: Appendix~\ref{app:runtime-calibration} reports the hardware inventory (Dawn CPU partition, workstation GPU, laptop CPU) and the cross-device calibration procedure. Per-method calibrated runtimes are listed in Table~\ref{tab:exp2-headtohead}. The LLM jailbreak experiments use a single GPU node for hidden-state extraction; the per-round runtimes are reported in Figure~\ref{fig:threshold-sweep-1e34}c.

\item {\bf Code Of Ethics}

    Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics?

    Answer: \answerYes{}

    Justification: The work uses public datasets (MNIST; JailbreakBench seeds) and standard published attack methods (PAIR) on publicly benchmarked models. No human-subjects research, no PII collection. The jailbreak experiments report only aggregate statistics, not adversarial prompts.

\item {\bf Broader Impacts}

    Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?

    Answer: \answerYes{}

    Justification: Section~\ref{sec:conclusion} notes that \projname\ enables cheaper, principled safety audits of rare failure modes (positive), but also acknowledges that more efficient failure-probability estimation could in principle inform adversarial discovery (negative). The framework operates at the population level (estimating failure probabilities) rather than producing individual adversarial inputs, which limits the direct misuse surface.

\item {\bf Safeguards}

    Question: Does the paper describe safeguards that have been put in place for responsible release of data or models with a high risk for misuse?

    Answer: \answerNA{}

    Justification: The main paper contains no adversarial prompts, jailbreak transcripts, or attack artefacts, and the submission releases no new pretrained models or scraped datasets; only an estimator framework, a ruler catalogue, and evaluation scripts. We note for the reviewers that the supplementary zipped repository includes instructions for regenerating PAIR- and GCG-style jailbreak records from public seeds and public model checkpoints; these instructions reuse already-published attack methods and do not redistribute attack prompts or jailbreak responses directly.

\item {\bf Licenses for existing assets}

    Question: Are the creators or original owners of assets used in the paper properly credited and are the license and terms of use explicitly mentioned and respected?

    Answer: \answerYes{}

    Justification: MNIST, JailbreakBench, PAIR, Llama-3.1-8B-Instruct, Qwen2.5-14B-Instruct, and Llama-Guard-3-8B are cited with their original publications. All are publicly available under their respective licenses and used within the terms of those licenses.

\item {\bf New Assets}

    Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?

    Answer: \answerYes{}

    Justification: The supplementary zipped repository ships the \projname\ reference implementation (ruler library, MNIST harness, LLM evaluation scripts) together with a README covering environment setup, dataset regeneration steps, and the runtime calibration procedure of Appendix~\ref{app:runtime-calibration}, plus a license file. No new datasets or pretrained models are introduced.

\item {\bf Crowdsourcing and Research with Human Subjects}

    Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation?

    Answer: \answerNA{}

    Justification: No crowdsourcing or human-subjects research.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}

    Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether IRB approvals were obtained?

    Answer: \answerNA{}

    Justification: No human subjects.

\item {\bf Declaration of LLM usage}

    Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?

    Answer: \answerYes{}

    Justification: Section~\ref{sec:exp-llm} applies \projname\ to LLM jailbreak probability estimation on three public LLMs (Llama-3.1-8B-Instruct as target, Qwen2.5-14B-Instruct as PAIR attacker, Llama-Guard-3-8B as safety judge). The LLM components are part of the experimental subject, not part of the estimator core: Section~\ref{sec:method} is model-agnostic.

\end{enumerate}

